Probing the dusty stellar populations of the Local Volume Galaxies with JWST/MIRI

The Mid-Infrared Instrument (MIRI) for the {\em James Webb Space Telescope} (JWST) will revolutionize our understanding of infrared stellar populations in the Local Volume. Using the rich {\em Spitzer}-IRS spectroscopic data-set and spectral classifications from the Surveying the Agents of Galaxy Evolution (SAGE)-Spectroscopic survey of over a thousand objects in the Magellanic Clouds, the Grid of Red supergiant and Asymptotic giant branch star ModelS ({\sc grams}), and the grid of YSO models by Robitaille et al. (2006), we calculate the expected flux-densities and colors in the MIRI broadband filters for prominent infrared stellar populations. We use these fluxes to explore the {\em JWST}/MIRI colours and magnitudes for composite stellar population studies of Local Volume galaxies. MIRI colour classification schemes are presented; these diagrams provide a powerful means of identifying young stellar objects, evolved stars and extragalactic background galaxies in Local Volume galaxies with a high degree of confidence. Finally, we examine which filter combinations are best for selecting populations of sources based on their JWST colours.

==> aasymbols.tex <==
% Astronomy and Astrophysics symbol macros (from aa.cls and mnras.cls)

\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}

\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}

\newcommand\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}

\newcommand\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\reset@font\scriptstyle\hat=$}}
{\hbox{$\reset@font\scriptscriptstyle\hat=$}}}}

\newcommand\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\newcommand\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\newcommand\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}

\newcommand\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}

\newcommand\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}

\newcommand\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}

\newcommand\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}

\newcommand\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}

\newcommand\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}

\newcommand\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\reset@font\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\reset@font\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}

\newcommand\sun{\hbox{$\odot$}}
\newcommand\earth{\hbox{$\oplus$}}
\newcommand\degr{\hbox{$^\circ$}}
\newcommand\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\reset@font\displaystyle/$}\hfil\crcr
{\hbox{$\reset@font\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\textstyle/$}\hfil\crcr
{\hbox{$\reset@font\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\scriptstyle/$}\hfil\crcr
{\hbox{$\reset@font\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\reset@font\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\reset@font\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\newcommand\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
\newcommand\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\newcommand{\romn}[1] {{\mathrm #1}}

%\newcommand\fd{\hbox{$.\!\!^{\reset@font\romn d}$}}
%\newcommand\fh{\hbox{$.\!\!^{\reset@font\romn h}$}}
%\newcommand\fm{\hbox{$.\!\!^{\reset@font\romn m}$}}
%\newcommand\fs{\hbox{$.\!\!^{\reset@font\romn s}$}}

\newcommand\fd{\hbox{$.\!\!^\mathrm{d}$}}
\newcommand\fh{\hbox{$.\!\!^\mathrm{h}$}}
\newcommand\fm{\hbox{$.\!\!^\mathrm{m}$}}
\newcommand\fs{\hbox{$.\!\!^\mathrm{s}$}}
\newcommand\fdg{\hbox{$.\!\!^\circ$}}
\newcommand\farcm{\hbox{$.\mkern-4mu^\prime$}}
\newcommand\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\newcommand\fp{\hbox{$.\!\!^{\reset@font\reset@font\scriptscriptstyle\romn p}$}}
\newcommand\arcdeg{\hbox{$^\circ$}}
\newcommand\arcmin{\hbox{$^\prime\,$}}
\newcommand\arcsec{\hbox{$^{\prime\prime}$}}

\def\micron{\hbox{$\umu$m}}


% end of definitions


==> journaldefs.tex <==
% bibliography and bibfile journal definitions (taken from aa.cls)

\def\aj{AJ}					% Astronomical Journal
\def\actaa{Acta Astron.}                        % Acta Astronomica
\def\araa{ARA\&A}				% Annual Review of Astron and Astrophys
\def\apj{ApJ}					% Astrophysical Journal
\def\apjl{ApJL}					% Astrophysical Journal, Letters
\def\apjs{ApJS}					% Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}				% Applied Optics
\def\apss{Ap\&SS}				% Astrophysics and Space Science
\def\aap{A\&A}					% Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}				% Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}				% Astronomy and Astrophysics, Supplement
\def\azh{AZh}					% Astronomicheskii Zhurnal
\def\baas{BAAS}					% Bulletin of the AAS
\def\jrasc{JRASC}				% Journal of the RAS of Canada
\def\memras{MmRAS}				% Memoirs of the RAS
\def\mnras{MNRAS}				% Monthly Notices of the RAS
\def\pra{Phys.~Rev.~A}				% Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}				% Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}				% Physical Review C
\def\prd{Phys.~Rev.~D}				% Physical Review D
\def\pre{Phys.~Rev.~E}				% Physical Review E
\def\prl{Phys.~Rev.~Lett.}			% Physical Review Letters
\def\pasp{PASP}					% Publications of the ASP
\def\pasj{PASJ}					% Publications of the ASJ
\def\qjras{QJRAS}				% Quarterly Journal of the RAS
\def\skytel{S\&T}				% Sky and Telescope
\def\solphys{Sol.~Phys.}			% Solar Physics
\def\sovast{Soviet~Ast.}			% Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}			% Space Science Reviews
\def\zap{ZAp}					% Zeitschrift fuer Astrophysik
\def\nat{Nature}				% Nature
\def\iaucirc{IAU~Circ.}				% IAU Cirulars
\def\aplett{Astrophys.~Lett.}			% Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}		% Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}	% Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}			% Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}		% Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}			% Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}			% Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}			% Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}	% Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}		% Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}			% Nuclear Physics A
\def\physrep{Phys.~Rep.}			% Physics Reports
\def\physscr{Phys.~Scr}				% Physica Scripta
\def\planss{Planet.~Space~Sci.}			% Planetary Space Science
\def\procspie{Proc.~SPIE}			% Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

% end of file



==> libbydefs.tex <==
% New Commands and Definitions

% Type styles

\newcommand{\sans}{\mdseries\sffamily\upshape}
\newcommand{\sansb}{\bfseries\sffamily\upshape}
\newcommand{\sansi}{\mdseries\sffamily\itshape}
\newcommand{\sansbi}{\bfseries\sffamily\itshape}
\newcommand{\sanssc}{\mdseries\sffamily\scshape}
\newcommand{\sansbsc}{\bfseries\sffamily\scshape}


% Units:

\newcommand{\cmpers}{\mbox{$\mathrm{cm\ s^{-1}}$}}
\newcommand{\cms}{\mbox{$\mathrm{cm^2}$}}
\newcommand{\cmspers}{\mbox{$\mathrm{cm^2\ s^{-1}}$}}
\newcommand{\ccpers}{\mbox{$\mathrm{cm^3\ s^{-1}}$}}
\newcommand{\percc}{\mbox{$\mathrm{cm^{-3}}$}}
\newcommand{\perccpers}{\mbox{$\mathrm{cm^{-3}\ s^{-1}}$}}
\newcommand{\kmpers}{\mbox{$\mathrm{km\ s^{-1}}$}}


% Various:

\newcommand{\zup}[1]{$^\mathrm{\,#1}$}
\newcommand{\x}{$\times$\ }
\newcommand{\etal}{\hbox{\it et al.\ }}
\newcommand{\ha}{H$\alpha$}
\newcommand{\ox}{[O{\sc iii}]}
\newcommand{\Av}{\mbox{$A_v$}}
\newcommand{\Ed}{\mbox{$E_\mathrm{D}$}}
\newcommand{\ISM}{\mbox{interstellar medium}}
\newcommand{\Vlsr}{\mbox{$V_\mathrm{LSR}$}}
\newcommand{\Lsol}{\hbox{L$_{\odot}$}}
\newcommand{\Msol}{\hbox{M$_{\odot}$}}
\newcommand{\Rsol}{\hbox{R$_{\odot}$}}


% Molecular Species:

\newcommand{\molh}{\mbox{$\mathrm{H_2}$}}
\newcommand{\Hp}{\mbox{$\mathrm{H^+}$}}
\newcommand{\Hep}{\mbox{$\mathrm{He^+}$}}
\newcommand{\HHHp}{\mbox{$\mathrm{H_3^+}$}}
\newcommand{\Cp}{\mbox{$\mathrm{C^+}$}}
\newcommand{\water}{\mbox{$\mathrm{H_2O}$}}
\newcommand{\CCH}{\mbox{$\mathrm{C_2H}$}}
\newcommand{\meth}{\mbox{$\mathrm{CH_3OH}$}}
\newcommand{\form}{\mbox{$\mathrm{H_2CO}$}}
\newcommand{\DDform}{\mbox{$\mathrm{D_2CO}$}}
\newcommand{\HCOp}{\mbox{$\mathrm{HCO^+}$}}
\newcommand{\ammo}{\mbox{$\mathrm{NH_3}$}}
\newcommand{\OO}{\mbox{$\mathrm{O_2}$}}
\newcommand{\HHD}{\mbox{$\mathrm{H_2D^+}$}}
\newcommand{\NNHp}{\mbox{$\mathrm{N_2H^+}$}}
\newcommand{\NND}{\hbox{N$_2$D$^+$}}


% Turbulence/Grains:

\newcommand{\Kz}{\mbox{$K=0$}}
\newcommand{\Ktwon}{\mbox{$K=10^{21}$}}
\newcommand{\Ktwtw}{\mbox{$K=10^{22}$}}
\newcommand{\Ktwth}{\mbox{$K=10^{23}$}}
\newcommand{\Tdis}{\mbox{$\tau_{dis}$}}
\newcommand{\Chieze}{Chi\`{e}ze}
\newcommand{\PdF}{Pineau des For\^{e}ts}
\newcommand{\vturb}{\mbox{$v_t$}}


% Objects:

%\newcommand{\IRAS}{\mbox{IRAS 16293-2422}}


% From Albert:

% \def\oversim#1#2{\lower0.5pt\vbox{\baselineskip0pt \lineskip-0.5pt 
%                  \ialign{$\mathsurround0pt #1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
% \def\gsim{\mathrel{\mathpalette\oversim>}}    % > over \sim
% \def\lsim{\mathrel{\mathpalette\oversim<}}    % < over \sim

% \newcommand{\note}[1]{{\bf [#1]}}

% note at end 
\def\thisrep{\vspace{0.5cm}\normalsize\noindent 
	     This report has been typeset from a \TeX\ / \LaTeX\ file prepared by the author.}
\def\thisshow{\vspace{0.5cm}\normalsize\noindent 
	     This slide show has been typeset from a \TeX\ / \LaTeX\ file prepared by the author.}

% end of file


